Ambiguity Analysis and Design of Sparse Arrays via Generalized Vandermonde Rank Conditions

Sparse linear arrays obtained by thinning a uniform linear array (ULA) achieve large effective apertures with a reduced number of physical sensors and have become a key enabling technology across radar, sonar, communications, and integrated sensing and communications. The price of thinning, however, is the emergence of ambiguities in the array manifold: distinct sets of directions of arrival that produce identical sensor measurements, precluding unique identification of multiple sources. Conventional sparse-array design criteria, based on beampattern shaping or estimation-performance optimization, do not fully capture how multiple steering vectors interact jointly to produce such ambiguities. This paper develops an algebraic framework for the complete multi-source identifiability analysis of thinned ULAs, characterizing all ambiguity sets for arbitrary source number rather than only at the maximum identifiable number. By relating the rank deficiency of the generalized Vandermonde matrix associated with the sparse steering matrix to that of a thinned Toeplitz matrix, and further to a rank condition on an augmented full-ULA steering matrix with prescribed generators, we obtain a systematic characterization of the ambiguity sets in large sparse arrays together with constructive design guidelines for ambiguity-free geometries. Algebraic and numerical examples demonstrate that the proposed framework resolves the ambiguity structure of thinned arrays of a few dozen grid positions, for which previous methods yield only individual ambiguity sets.

==> matrixmacros_modernized.tex <==
\usetikzlibrary{positioning, calc, decorations.pathreplacing, arrows.meta, fit}

\definecolor{brightyellow}{HTML}{FFFF00}
\definecolor{red}{HTML}{FF0000}
\colorlet{lightyellow}{brightyellow!75!white}
\colorlet{lightgreen}{green!55!white}
\colorlet{darkgreen}{green!45!black}
\colorlet{lightblue}{blue!35!white}
\colorlet{lightteal}{teal!45!white}
\colorlet{cyanshift}{cyan!80!blue}

\def\gridsize{3mm}
\def\dimamount{35}
\def\dimcolor{gray!45}

% ---------- global "modern" style tokens ----------
% Tune these once to restyle every matrix diagram consistently.
\def\cellradius{0.35mm}      % corner rounding on individual cells
\def\cellshrink{0.80}        % drawn cell size = \cellshrink * grid pitch (creates the gap)
\def\bordercolor{black!45}   % cell stroke color (soft, not pure black)
\def\frameradius{1.6pt}      % corner rounding on the outer "matrix" frame
\def\framepad{0.20}          % extra frame padding beyond cells, in units of grid pitch
\def\framecolor{black!55}    % outer frame stroke color

% Outer frame is only drawn when the node's fill resolves to literal "white":
% colored data matrices rely on their fill color as the visual boundary,
% while white/sparse structural nodes (selection matrices, mixed columns)
% get a frame so they don't disappear against the panel background.
\newcommand{\isexactlywhite}[1]{%
  \def\whitetoken{white}%
  \edef\tmpcolortest{#1}%
  \ifx\tmpcolortest\whitetoken
  \def\iswhiteresult{1}%
  \else
  \def\iswhiteresult{0}%
  \fi
}

\newlength{\eqbbNorthY}
\newlength{\eqbbSouthY}
\newlength{\STy}

\newcommand{\equalizearound}[1]{%
  \pgfextracty{\eqbbNorthY}{\pgfpointanchor{current bounding box}{north}}%
  \pgfextracty{\eqbbSouthY}{\pgfpointanchor{current bounding box}{south}}%
  \pgfmathsetlengthmacro{\eqgapN}{\eqbbNorthY-(#1)}%
  \pgfmathsetlengthmacro{\eqgapS}{(#1)-\eqbbSouthY}%
  \pgfmathsetlengthmacro{\eqgapMax}{max(\eqgapN,\eqgapS)}%
  \path ({0},{(#1)+\eqgapMax}) ({0},{(#1)-\eqgapMax});%
}

\newcommand{\isinlist}[2]{%
  \def\inlistresult{0}%
  \edef\isinlisttest{#2}%
  \ifx\isinlisttest\empty
  \else
  \foreach \ilt in #2{ \ifnum\ilt=#1 \xdef\inlistresult{1}\fi }%
  \fi
}

\newcommand{\colorgridrowsnode}[6][]{%
  \begingroup
  \pgfkeys{/cg/.cd, size/.initial=\gridsize, base/.initial=brightyellow,
    shift/.initial=red, rowmax/.initial=100, colmax/.initial=65,
    border/.initial=0.5pt, outerborder/.initial=0.7pt,
    cellradius/.initial=\cellradius, cellshrink/.initial=\cellshrink,
    bordercolor/.initial=\bordercolor, frameradius/.initial=\frameradius,
    framepad/.initial=\framepad, framecolor/.initial=\framecolor,
  dimrows/.initial={}, dimamount/.initial=\dimamount, dimcolor/.initial=\dimcolor, #1}
  \pgfkeysgetvalue{/cg/size}{\S}
  \pgfkeysgetvalue{/cg/base}{\B}
  \pgfkeysgetvalue{/cg/shift}{\Sh}
  \pgfkeysgetvalue{/cg/rowmax}{\RM}
  \pgfkeysgetvalue{/cg/colmax}{\CM}
  \pgfkeysgetvalue{/cg/border}{\Bd}
  \pgfkeysgetvalue{/cg/outerborder}{\OB}
  \pgfkeysgetvalue{/cg/cellradius}{\CR}
  \pgfkeysgetvalue{/cg/cellshrink}{\CSk}
  \pgfkeysgetvalue{/cg/bordercolor}{\BC}
  \pgfkeysgetvalue{/cg/frameradius}{\FR}
  \pgfkeysgetvalue{/cg/framepad}{\FP}
  \pgfkeysgetvalue{/cg/framecolor}{\FC}
  \pgfkeysgetvalue{/cg/dimrows}{\DR}
  \pgfkeysgetvalue{/cg/dimamount}{\DA}
  \pgfkeysgetvalue{/cg/dimcolor}{\DC}
  \pgfmathsetmacro{\rd}{max(#5-1,1)}
  \pgfmathsetmacro{\cd}{max(#6-1,1)}
  \isexactlywhite{\B}\let\isBwhite\iswhiteresult
  \isexactlywhite{\Sh}\let\isShwhite\iswhiteresult
  \def\CBd{none}%
  \ifnum\isBwhite=1 \ifnum\isShwhite=1 \def\CBd{\BC}\fi\fi
  \xdef\lastpos{0}
  \foreach \k [count=\pos from 0] in {#4}{ \xdef\lastpos{\pos} }
  \pgfmathsetmacro{\nsel}{\lastpos+1}
  \pgfmathsetlengthmacro{\W}{#6*\S}
  \pgfmathsetlengthmacro{\Ht}{\nsel*\S}
  \pgfmathsetlengthmacro{\CS}{\CSk*\S}
  \node[minimum width=\W, minimum height=\Ht, inner sep=0pt, outer sep=0pt, #3] (#2) {};
  \coordinate (origin-#2) at ($(#2.north west)+(0.5*\S,-0.5*\S)$);
  \begin{scope}[shift={(origin-#2)}]
    \xdef\lastpos{0}
    \foreach \k [count=\pos from 0] in {#4}{
      \isinlist{\k}{\DR}
      \edef\rowdim{\inlistresult}
      \foreach \j in {1,...,#6}{
        \pgfmathsetmacro{\yp}{100-((\k-1)/\rd)*\RM}
        \pgfmathsetmacro{\cp}{100-((\j-1)/\cd)*\CM}
        \colorlet{cellcolor}{\B!\yp!\Sh!\cp!white}
        \ifnum\rowdim=1
        \pgfmathsetmacro{\keeppct}{100-\DA}
        \colorlet{cellcolor}{cellcolor!\keeppct!\DC}
        \fi
        \node[draw=\CBd, line width=\Bd, rounded corners=\CR, fill=cellcolor,
        minimum size=\CS, inner sep=0pt]
        at ({(\j-1)*\S},{-\pos*\S}) {};
      }
      \xdef\lastpos{\pos}
    }
    \draw[draw=\FC, line width=\OB, rounded corners=\FR]
    ({-(0.5+\FP)*\S},{(0.5+\FP)*\S}) rectangle ({(#6-1+0.5+\FP)*\S},{-(\nsel-1+0.5+\FP)*\S});
  \end{scope}
  \endgroup
}

\newcommand{\colorgridnode}[5][]{%
  \colorgridrowsnode[#1]{#2}{#3}{1,...,#4}{#4}{#5}%
}

\newcommand{\selectionmatrixnode}[5][]{%
  \begingroup
  \pgfkeys{/sm/.cd, size/.initial=\gridsize, color/.initial=gray!60,
    border/.initial=0.5pt, outerborder/.initial=0.7pt,
    cellradius/.initial=\cellradius, cellshrink/.initial=\cellshrink,
    bordercolor/.initial=\bordercolor, frameradius/.initial=\frameradius,
  framepad/.initial=\framepad, framecolor/.initial=\framecolor, #1}
  \pgfkeysgetvalue{/sm/size}{\S}
  \pgfkeysgetvalue{/sm/color}{\C}
  \pgfkeysgetvalue{/sm/border}{\Bd}
  \pgfkeysgetvalue{/sm/outerborder}{\OB}
  \pgfkeysgetvalue{/sm/cellradius}{\CR}
  \pgfkeysgetvalue{/sm/cellshrink}{\CSk}
  \pgfkeysgetvalue{/sm/bordercolor}{\BC}
  \pgfkeysgetvalue{/sm/frameradius}{\FR}
  \pgfkeysgetvalue{/sm/framepad}{\FP}
  \pgfkeysgetvalue{/sm/framecolor}{\FC}
  \isexactlywhite{\C}\let\isCwhite\iswhiteresult
  \def\CBd{none}%
  \ifnum\isCwhite=1 \def\CBd{\BC}\fi
  \xdef\lastpos{0}
  \foreach \k [count=\pos from 0] in {#4}{ \xdef\lastpos{\pos} }
  \pgfmathsetmacro{\nsel}{\lastpos+1}
  \pgfmathsetlengthmacro{\W}{#5*\S}
  \pgfmathsetlengthmacro{\Ht}{\nsel*\S}
  \pgfmathsetlengthmacro{\CS}{\CSk*\S}
  \node[minimum width=\W, minimum height=\Ht, inner sep=0pt, outer sep=0pt, #3] (#2) {};
  \coordinate (origin-#2) at ($(#2.north west)+(0.5*\S,-0.5*\S)$);
  \begin{scope}[shift={(origin-#2)}]
    \xdef\lastpos{0}
    \foreach \k [count=\pos from 0] in {#4}{
      \node[draw=\CBd, line width=\Bd, rounded corners=\CR, fill=\C,
      minimum size=\CS, inner sep=0pt]
      at ({(\k-1)*\S},{-\pos*\S}) {};
      \xdef\lastpos{\pos}
    }
    \draw[draw=\FC, line width=\OB, rounded corners=\FR]
    ({-(0.5+\FP)*\S},{(0.5+\FP)*\S}) rectangle ({(#5-1+0.5+\FP)*\S},{-(\nsel-1+0.5+\FP)*\S});
  \end{scope}
  \endgroup
}

\newcommand{\selectiontransposenode}[5][]{%
  \begingroup
  \pgfkeys{/st/.cd, size/.initial=\gridsize, color/.initial=gray!60,
    border/.initial=0.5pt, outerborder/.initial=0.7pt,
    cellradius/.initial=\cellradius, cellshrink/.initial=\cellshrink,
    bordercolor/.initial=\bordercolor, frameradius/.initial=\frameradius,
  framepad/.initial=\framepad, framecolor/.initial=\framecolor, #1}
  \pgfkeysgetvalue{/st/size}{\S}
  \pgfkeysgetvalue{/st/color}{\C}
  \pgfkeysgetvalue{/st/border}{\Bd}
  \pgfkeysgetvalue{/st/outerborder}{\OB}
  \pgfkeysgetvalue{/st/cellradius}{\CR}
  \pgfkeysgetvalue{/st/cellshrink}{\CSk}
  \pgfkeysgetvalue{/st/bordercolor}{\BC}
  \pgfkeysgetvalue{/st/frameradius}{\FR}
  \pgfkeysgetvalue{/st/framepad}{\FP}
  \pgfkeysgetvalue{/st/framecolor}{\FC}
  \isexactlywhite{\C}\let\isCwhite\iswhiteresult
  \def\CBd{none}%
  \ifnum\isCwhite=1 \def\CBd{\BC}\fi
  \xdef\lastidx{0}
  \foreach \r [count=\idx from 1] in {#4}{ \xdef\lastidx{\idx} }
  \pgfmathsetmacro{\nsel}{\lastidx}
  \pgfmathsetlengthmacro{\W}{\nsel*\S}
  \pgfmathsetlengthmacro{\Ht}{#5*\S}
  \pgfmathsetlengthmacro{\CS}{\CSk*\S}
  \node[minimum width=\W, minimum height=\Ht, inner sep=0pt, outer sep=0pt, #3] (#2) {};
  \coordinate (origin-#2) at ($(#2.north west)+(0.5*\S,-0.5*\S)$);
  \begin{scope}[shift={(origin-#2)}]
    \foreach \r [count=\idx from 1] in {#4}{
      \node[draw=\CBd, line width=\Bd, rounded corners=\CR, fill=\C,
      minimum size=\CS, inner sep=0pt]
      at ({(\idx-1)*\S},{-(\r-1)*\S}) {};
    }
    \draw[draw=\FC, line width=\OB, rounded corners=\FR]
    ({-(0.5+\FP)*\S},{(0.5+\FP)*\S}) rectangle ({(\nsel-1+0.5+\FP)*\S},{-(#5-1+0.5+\FP)*\S});
  \end{scope}
  \endgroup
}

\newcommand{\mixedcolumnnode}[5][]{%
  \begingroup
  \pgfkeys{/mc/.cd, size/.initial=\gridsize, base/.initial=brightyellow,
    shift/.initial=red, rowmax/.initial=100, border/.initial=0.5pt,
    outerborder/.initial=0.7pt, empty/.initial=white,
    cellradius/.initial=\cellradius, cellshrink/.initial=\cellshrink,
    bordercolor/.initial=\bordercolor, frameradius/.initial=\frameradius,
  framepad/.initial=\framepad, framecolor/.initial=\framecolor, #1}
  \pgfkeysgetvalue{/mc/size}{\S}
  \pgfkeysgetvalue{/mc/base}{\B}
  \pgfkeysgetvalue{/mc/shift}{\Sh}
  \pgfkeysgetvalue{/mc/rowmax}{\RM}
  \pgfkeysgetvalue{/mc/border}{\Bd}
  \pgfkeysgetvalue{/mc/outerborder}{\OB}
  \pgfkeysgetvalue{/mc/empty}{\Em}
  \pgfkeysgetvalue{/mc/cellradius}{\CR}
  \pgfkeysgetvalue{/mc/cellshrink}{\CSk}
  \pgfkeysgetvalue{/mc/bordercolor}{\BC}
  \pgfkeysgetvalue{/mc/frameradius}{\FR}
  \pgfkeysgetvalue{/mc/framepad}{\FP}
  \pgfkeysgetvalue{/mc/framecolor}{\FC}
  \isexactlywhite{\Em}\let\isEmwhite\iswhiteresult
  \def\EBd{none}%
  \ifnum\isEmwhite=1 \def\EBd{\BC}\fi
  \isexactlywhite{\B}\let\isBwhite\iswhiteresult
  \isexactlywhite{\Sh}\let\isShwhite\iswhiteresult
  \def\HBd{none}%
  \ifnum\isBwhite=1 \ifnum\isShwhite=1 \def\HBd{\BC}\fi\fi
  \pgfmathsetlengthmacro{\W}{\S}
  \pgfmathsetlengthmacro{\Ht}{#4*\S}
  \pgfmathsetlengthmacro{\CS}{\CSk*\S}
  \node[minimum width=\W, minimum height=\Ht, inner sep=0pt, outer sep=0pt, #3] (#2) {};
  \coordinate (origin-#2) at ($(#2.north west)+(0.5*\S,-0.5*\S)$);
  \begin{scope}[shift={(origin-#2)}]
    \def\HL{#5}%
    \foreach \r in {1,...,#4}{
      \isinlist{\r}{\HL}
      \ifnum\inlistresult=0
      \node[draw=\EBd, line width=\Bd, rounded corners=\CR, fill=\Em,
      minimum size=\CS, inner sep=0pt]
      at (0,{-(\r-1)*\S}) {};
      \fi
    }
    \xdef\lastidx{0}
    \foreach \r [count=\idx from 1] in {#5}{ \xdef\lastidx{\idx} }
    \pgfmathsetmacro{\nf}{\lastidx}
    \pgfmathsetmacro{\rd}{max(\nf-1,1)}
    \foreach \r [count=\idx from 1] in {#5}{
      \pgfmathsetmacro{\yp}{100-((\idx-1)/\rd)*\RM}
      \colorlet{cellcolor}{\B!\yp!\Sh}
      \node[draw=\HBd, line width=\Bd, rounded corners=\CR, fill=cellcolor,
      minimum size=\CS, inner sep=0pt]
      at (0,{-(\r-1)*\S}) {};
    }
    \draw[draw=\FC, line width=\OB, rounded corners=\FR]
    ({-(0.5+\FP)*\S},{(0.5+\FP)*\S}) rectangle ({(0.5+\FP)*\S},{-(#4-1+0.5+\FP)*\S});
  \end{scope}
  \endgroup
}

\newcommand{\toeplitznode}[6][]{%
  \begingroup
  \pgfkeys{/tz/.cd, size/.initial=\gridsize, rowbase/.initial=blue,
    rowshift/.initial=violet, colmax/.initial=85,
    border/.initial=0.5pt, outerborder/.initial=0.7pt,
    keepcols/.initial={}, dimamount/.initial=\dimamount, dimcolor/.initial=\dimcolor,
    cellradius/.initial=\cellradius, cellshrink/.initial=\cellshrink,
    bordercolor/.initial=\bordercolor, frameradius/.initial=\frameradius,
  framepad/.initial=\framepad, framecolor/.initial=\framecolor, #1}
  \pgfkeysgetvalue{/tz/size}{\S}
  \pgfkeysgetvalue{/tz/rowbase}{\RB}
  \pgfkeysgetvalue{/tz/rowshift}{\RS}
  \pgfkeysgetvalue{/tz/colmax}{\CM}
  \pgfkeysgetvalue{/tz/border}{\Bd}
  \pgfkeysgetvalue{/tz/outerborder}{\OB}
  \pgfkeysgetvalue{/tz/keepcols}{\KC}
  \pgfkeysgetvalue{/tz/dimamount}{\DA}
  \pgfkeysgetvalue{/tz/dimcolor}{\DC}
  \pgfkeysgetvalue{/tz/cellradius}{\CR}
  \pgfkeysgetvalue{/tz/cellshrink}{\CSk}
  \pgfkeysgetvalue{/tz/bordercolor}{\BC}
  \pgfkeysgetvalue{/tz/frameradius}{\FR}
  \pgfkeysgetvalue{/tz/framepad}{\FP}
  \pgfkeysgetvalue{/tz/framecolor}{\FC}
  \isexactlywhite{\RB}\let\isRBwhite\iswhiteresult
  \isexactlywhite{\RS}\let\isRSwhite\iswhiteresult
  \def\CBd{none}%
  \ifnum\isRBwhite=1 \ifnum\isRSwhite=1 \def\CBd{\BC}\fi\fi
  \pgfmathsetmacro{\rd}{max(#4-1,1)}
  \pgfmathsetmacro{\bd}{max(#6-1,1)}
  \pgfmathsetlengthmacro{\W}{#5*\S}
  \pgfmathsetlengthmacro{\Ht}{#4*\S}
  \pgfmathsetlengthmacro{\CS}{\CSk*\S}
  \node[minimum width=\W, minimum height=\Ht, inner sep=0pt, outer sep=0pt, #3] (#2) {};
  \coordinate (origin-#2) at ($(#2.north west)+(0.5*\S,-0.5*\S)$);
  \begin{scope}[shift={(origin-#2)}]
    \foreach \r in {1,...,#4}{
      \pgfmathsetmacro{\rp}{100-((\r-1)/\rd)*100}
      \colorlet{rowcolor}{\RB!\rp!\RS}
      \foreach \b in {1,...,#6}{
        \pgfmathsetmacro{\j}{\r+\b-1}
        \pgfmathsetmacro{\cp}{100-((\b-1)/\bd)*\CM}
        \colorlet{cellcolor}{rowcolor!\cp!white}
        \edef\kctest{\KC}
        \ifx\kctest\empty
        \else
        \isinlist{\j}{\KC}
        \ifnum\inlistresult=0
        \pgfmathsetmacro{\keeppct}{100-\DA}
        \colorlet{cellcolor}{cellcolor!\keeppct!\DC}
        \fi
        \fi
        \node[draw=\CBd, line width=\Bd, rounded corners=\CR, fill=cellcolor,
        minimum size=\CS, inner sep=0pt]
        at ({(\j-1)*\S},{-(\r-1)*\S}) {};
      }
    }
    \draw[draw=\FC, line width=\OB, rounded corners=\FR]
    ({-(0.5+\FP)*\S},{(0.5+\FP)*\S}) rectangle ({(#5-1+0.5+\FP)*\S},{-(#4-1+0.5+\FP)*\S});
  \end{scope}
  \endgroup
}

\newcommand{\toeplitzcolsnode}[6][]{%
  \begingroup
  \pgfkeys{/tzc/.cd, size/.initial=\gridsize, rowbase/.initial=darkgreen,
    rowshift/.initial=darkgreen, colmax/.initial=85,
    border/.initial=0.5pt, outerborder/.initial=0.7pt,
    cellradius/.initial=\cellradius, cellshrink/.initial=\cellshrink,
    bordercolor/.initial=\bordercolor, frameradius/.initial=\frameradius,
  framepad/.initial=\framepad, framecolor/.initial=\framecolor, #1}
  \pgfkeysgetvalue{/tzc/size}{\S}
  \pgfkeysgetvalue{/tzc/rowbase}{\RB}
  \pgfkeysgetvalue{/tzc/rowshift}{\RS}
  \pgfkeysgetvalue{/tzc/colmax}{\CM}
  \pgfkeysgetvalue{/tzc/border}{\Bd}
  \pgfkeysgetvalue{/tzc/outerborder}{\OB}
  \pgfkeysgetvalue{/tzc/cellradius}{\CR}
  \pgfkeysgetvalue{/tzc/cellshrink}{\CSk}
  \pgfkeysgetvalue{/tzc/bordercolor}{\BC}
  \pgfkeysgetvalue{/tzc/frameradius}{\FR}
  \pgfkeysgetvalue{/tzc/framepad}{\FP}
  \pgfkeysgetvalue{/tzc/framecolor}{\FC}
  \isexactlywhite{\RB}\let\isRBwhite\iswhiteresult
  \isexactlywhite{\RS}\let\isRSwhite\iswhiteresult
  \def\CBd{none}%
  \ifnum\isRBwhite=1 \ifnum\isRSwhite=1 \def\CBd{\BC}\fi\fi
  \pgfmathsetmacro{\rd}{max(#5-1,1)}
  \pgfmathsetmacro{\bd}{max(#6-1,1)}
  \xdef\lastidx{0}
  \foreach \j [count=\idx from 1] in {#4}{ \xdef\lastidx{\idx} }
  \pgfmathsetmacro{\ncols}{\lastidx}
  \pgfmathsetlengthmacro{\W}{\ncols*\S}
  \pgfmathsetlengthmacro{\Ht}{#5*\S}
  \pgfmathsetlengthmacro{\CS}{\CSk*\S}
  \node[minimum width=\W, minimum height=\Ht, inner sep=0pt, outer sep=0pt, #3] (#2) {};
  \coordinate (origin-#2) at ($(#2.north west)+(0.5*\S,-0.5*\S)$);
  \begin{scope}[shift={(origin-#2)}]
    \foreach \r in {1,...,#5}{
      \pgfmathsetmacro{\rp}{100-((\r-1)/\rd)*100}
      \colorlet{rowcolor}{\RB!\rp!\RS}
      \foreach \j [count=\idx from 1] in {#4}{
        \pgfmathsetmacro{\b}{\j-\r+1}
        \ifdim\b pt>0.5pt
        \pgfmathparse{\b<=#6 ? 1 : 0}
        \ifdim\pgfmathresult pt>0.5pt
        \pgfmathsetmacro{\cp}{100-((\b-1)/\bd)*\CM}
        \colorlet{cellcolor}{rowcolor!\cp!white}
        \node[draw=\CBd, line width=\Bd, rounded corners=\CR, fill=cellcolor,
        minimum size=\CS, inner sep=0pt]
        at ({(\idx-1)*\S},{-(\r-1)*\S}) {};
        \fi
        \fi
      }
    }
    \draw[draw=\FC, line width=\OB, rounded corners=\FR]
    ({-(0.5+\FP)*\S},{(0.5+\FP)*\S}) rectangle ({(\ncols-1+0.5+\FP)*\S},{-(#5-1+0.5+\FP)*\S});
  \end{scope}
  \endgroup
}

==> panel1_rank_deficient.tex <==
% \documentclass[tikz]{standalone}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \input{matrixmacros.tex}
% \begin{document}
\centering
\begin{tikzpicture}\footnotesize
  \colorgridrowsnode[base=lightyellow]{AI}{at={(0,0)}, anchor=east}%
  {1,3,4,7,8}{8}{4}
  \node[above=2mm of AI] {$\boldsymbol{A}_{\mathcal{I}}$};

  \colorgridnode[base=cyanshift, shift=lightteal]{x1}{anchor=west, right=2mm of AI.east}{4}{1}
  \node[above=2mm of x1] {$\boldsymbol{x}$};

  \node[anchor=west, right=2mm of x1.east] (eq) {$=$};

  \selectionmatrixnode{S}{anchor=west, right=2mm of eq.east}{1,3,4,7,8}{8}
  \node[above=2mm of S] {$\boldsymbol{T}_{\mathcal{I}}$};

  \colorgridnode[base=lightyellow, dimrows={2,5,6}]{AM}{anchor=west, right=2mm of S.east}{8}{4}
  \node[above=2mm of AM] {$\boldsymbol{A}_M$};

  \colorgridnode[base=cyanshift, shift=lightteal]{x2}{anchor=west, right=2mm of AM.east}{4}{1}
  \node[above=2mm of x2] {$\boldsymbol{x}$};

  \coordinate (braceA-left)  at ($(AI.south west)+(0,-4pt)$);
  \coordinate (braceA-right) at ($(x1.south east |- AI.south)+(0,-4pt)$);
  \draw[decorate, decoration={brace, amplitude=5pt, mirror}]
  (braceA-left) -- (braceA-right) node[midway, below=5pt] {$\boldsymbol{y}_{\mathcal{I}} = \boldsymbol{0}$};

  \coordinate (braceM-left)  at ($(AM.south west)+(0,-4pt)$);
  \coordinate (braceM-right) at ($(x2.south east |- AM.south)+(0,-4pt)$);
  \draw[decorate, decoration={brace, amplitude=5pt, mirror}]
  (braceM-left) -- (braceM-right) node[midway, below=5pt] {$\boldsymbol{y}_M \in \mathcal{R}(\boldsymbol{A}_M)$};

  % \node[above=0pt of current bounding box.north, align=center]
  % {$\boldsymbol{A}_{\mathcal{I}}(z_1,\ldots, z_L)$ is rank deficient $\Leftrightarrow$ there exist a \blue{nullspace vector} ${\boldsymbol x}$ such that ${\boldsymbol y}_{\mathcal I} = {\boldsymbol A}_{\mathcal I}{\boldsymbol x}={\boldsymbol 0}$.};
  % \equalizearound{0pt}
\end{tikzpicture}
% \end{document}

==> panel2_inflate.tex <==
% \documentclass[tikz]{standalone}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \input{matrixmacros.tex}
% \begin{document}
\centering
\begin{tikzpicture}\footnotesize
  \colorgridnode[base=lightblue, shift=violet]{Vtop}{at={(0,0)}, anchor=north}{3}{1}
  \node[above=2mm of Vtop] {$\boldsymbol{y}_{\bar{\mathcal{I}}} = \boldsymbol{A}_{\bar{\mathcal{I}}}\boldsymbol{x}$};
  \node[anchor=west, right=2mm of Vtop.east] (neq0) {$\neq \boldsymbol{0}$};

  \colorgridnode[base=white, shift=white]{Vbot}{anchor=north, below=3mm of Vtop.south}{5}{1}
  \node[below=2mm of Vbot] {$\boldsymbol{y}_{\mathcal{I}} = \boldsymbol{A}_{\mathcal{I}}\boldsymbol{x}$};
  \node[anchor=west, right=2mm of Vbot.east] (eq0) {$=\boldsymbol{0}$};

  \coordinate (stackmid) at ($(Vtop.north)!0.5!(Vbot.south)$);

  \mixedcolumnnode[base=lightblue, shift=violet]{Ycomb}%
  {at={($(Vtop.east |- stackmid)+(20mm,0)$)}, anchor=west}{8}{2,5,6}
  \node[above=2mm of Ycomb] {$\boldsymbol{y}_M\!\in\! {\mathcal R}\big( {\boldsymbol A}_M \big)$};

  \draw[-{Stealth[length=6pt]}, shorten >=5mm, shorten <=4mm]
  (neq0.east) -- (Ycomb.west);
  \draw[-{Stealth[length=6pt]}, shorten >=4mm, shorten <=4mm]
  (eq0.east) -- (Ycomb.west);

  \node[anchor=west, right=2mm of Ycomb.east] (eq2) {$=$};

  \selectiontransposenode{ST}{anchor=west, right=2mm of eq2.east}{2,5,6}{8}
  \node[above=2mm of ST] {$\boldsymbol{T}_{\bar{\mathcal{I}}}^{\top}$};

  \colorgridnode[base=lightblue, shift=violet]{Vtop2}{anchor=west, right=2mm of ST.east}{3}{1}
  \node[above=2mm of Vtop2] {$\boldsymbol{y}_{\bar{\mathcal{I}}}$};

  % \node[above=0pt of current bounding box.north, align=center]
  % {$\boldsymbol{y}_M$ can be inflated from \blue{auxiliary data} (virtual measurements)  $\boldsymbol{y}_{\bar{\mathcal{I}}}$.};
  % \pgfextracty{\STy}{\pgfpointanchor{ST}{center}}%
  % \equalizearound{\STy}
\end{tikzpicture}
% \end{document}

==> panel3_toeplitz_y_null.tex <==
% \documentclass[tikz]{standalone}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \input{matrixmacros.tex}
% \begin{document}
\centering
\begin{tikzpicture}\footnotesize
  \toeplitznode[rowbase=darkgreen, rowshift=darkgreen, keepcols={2,5,6}]{Tz}%
  {at={(0,0)}, anchor=east}{4}{8}{5}
  \node[above=2mm of Tz] {$\mathcal{T}(\boldsymbol{g})$};

  \mixedcolumnnode[base=lightblue, shift=violet]{Yvec}{anchor=west, right=2mm of Tz.east}{8}{2,5,6}
  \node[above=2mm of Yvec,xshift=2mm] {$\boldsymbol{y}_M \in {\mathcal R}\big( {\boldsymbol A}_M \big)$};

  \node[anchor=west, right=2mm of Yvec.east] (eqTz) {$=$};
  \node[anchor=west, right=0mm of eqTz.east] {$\boldsymbol{0}$};

  % \node[above=5pt of current bounding box.north, align=center]
  % {$\mathcal{T}(\boldsymbol{g}) \boldsymbol{y}_M = \mathcal{T}(\boldsymbol{g}) \boldsymbol{A}_M \boldsymbol{x} = \boldsymbol{0}$ since $\mathcal{R}(\boldsymbol{A}_M) = \mathcal{N}\left(\mathcal{T}(\boldsymbol{g})\right)$.};
\end{tikzpicture}
% \end{document}

==> panel4_toeplitz_cols.tex <==
% \documentclass[tikz]{standalone}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \input{matrixmacros.tex}
% \begin{document}
\centering
\begin{tikzpicture}\footnotesize
  \toeplitzcolsnode[rowbase=darkgreen, rowshift=darkgreen]{TzCols}{at={(0,0)}, anchor=west}{2,5,6}{4}{5}
  \node[above=2mm of TzCols] {$\mathcal{T}_{\bar{\mathcal{I}}}(\boldsymbol{g})$};

  \colorgridnode[base=lightblue, shift=violet]{YIbar2}{anchor=west, right=2mm of TzCols.east}{3}{1}
  \node[above=2mm of YIbar2] {$\boldsymbol{y}_{\bar{\mathcal{I}}}$};

  \node[anchor=west, right=2mm of YIbar2.east] (eqbang) {$=$};
  \node[anchor=west, right=0mm of eqbang.east] {$\boldsymbol{0}$};

  % \node[above=5pt of current bounding box.north, align=center]
  % {$\mathcal{T}_{\bar{\mathcal{I}}}(\boldsymbol{g})$ is \blue{rank deficient}.};
\end{tikzpicture}
% \end{document}
